CitySTAR: Structured and Topology-Aware Reasoning for Open-Vocabulary Urban 3D Grounding

3D grounding aims to localize target entities in complex scenes from natural language and plays a fundamental role in embodied perception and spatial reasoning. However, existing approaches mostly rely on feature similarity or direct matching, making it difficult to connect natural-language intent with the implicit semantic and geometric structures hidden in billion-scale urban point clouds. We reformulate city-scale 3D grounding as structured constraint reasoning, where description semantics are organized into computable cross-modal constraints over open-vocabulary 3D entities, attributes, and spatial relations. We present CitySTAR, a training-free framework for reasoning-driven urban 3D grounding. CitySTAR lifts raw billion-scale urban point clouds into a query-ready scene graph of open-vocabulary 3D instances, with CodeLLM-driven tools supplying multimodal evidence for node attributes and 3D spatial relations. It then models target-context topology with paired hypergraphs and performs bidirectional topology verification for structural disambiguation. Finally, a Reflective Cross-modal Grounding module integrates topology consistency and candidate-centered 2D visual evidence to make decisions over a metric-aware 3D context graph. To further support this setting, we introduce CitySTAR-3D, an enhanced benchmark that improves semantic coverage, instance completeness, bounding-box fidelity, and spatial-relation complexity in city-scale 3D grounding. Extensive experiments show that CitySTAR consistently improves open-world urban 3D grounding while maintaining strong interpretability and generalization.

==> sections/discussion.tex <==
\section{Data}
\label{sec:data}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.92\linewidth]{pngs/image2.png}
  \caption{\textbf{Data pipeline.} Replace this placeholder with a dataset construction, preprocessing, or annotation workflow.}
  \label{fig:data_pipeline}
\end{figure*}

Describe the data sources, collection protocol, filtering criteria, annotation process, and dataset splits.
Include enough detail for readers to understand the scope and limitations of the data without exposing private or unreleased information.

\textbf{Collection.}
Explain where the data comes from and what inclusion criteria were applied.
If applicable, report the number of samples, domains, classes, annotators, or acquisition devices.

\textbf{Preprocessing.}
Describe cleaning, normalization, deduplication, quality control, and format conversion.
Reference Figure~\ref{fig:data_pipeline} if the pipeline is shown visually.

\textbf{Splits and Usage.}
State how training, validation, and test splits are constructed.
Mention measures taken to prevent leakage between splits.

\textbf{Ethics and Licensing.}
Summarize consent, privacy, licensing, and safety considerations when they apply.
For public datasets, cite the original sources, such as a placeholder reference~\cite{sample_reference}.

